Broaden the Vision: Geo-Diverse Visual Commonsense Reasoning

Commonsense is defined as the knowledge that is shared by everyone. However, certain types of commonsense knowledge are correlated with culture and geographic locations and they are only shared locally. For example, the scenarios of wedding ceremonies vary across regions due to different customs influenced by historical and religious factors. Such regional characteristics, however, are generally omitted in prior work. In this paper, we construct a Geo-Diverse Visual Commonsense Reasoning dataset (GD-VCR) to test vision-and-language models' ability to understand cultural and geo-location-specific commonsense. In particular, we study two state-of-the-art Vision-and-Language models, VisualBERT and ViLBERT trained on VCR, a standard multimodal commonsense benchmark with images primarily from Western regions. We then evaluate how well the trained models can generalize to answering the questions in GD-VCR. We find that the performance of both models for non-Western regions including East Asia, South Asia, and Africa is significantly lower than that for Western region. We analyze the reasons behind the performance disparity and find that the performance gap is larger on QA pairs that: 1) are concerned with culture-related scenarios, e.g., weddings, religious activities, and festivals; 2) require high-level geo-diverse commonsense reasoning rather than low-order perception and recognition. Dataset and code are released at https://github.com/WadeYin9712/GD-VCR.

==> newref.tex <==
% The file contains papers cited by UCLA-NLP Group that are not in nlp.bib and ref.bib
% Only published papers should be included in this file. 
% For Arxiv, please add them to preprint.bib
% Papers published at NLP venues have been automatically added to nlp.bib. 
% Therefore, please only include papers published in other venues here.
% The entries added in this bibfile will be merge to ref.bib later.
% Check 0-Readme.tex for the format of bib entries. 

@STRING{aaai	= {Proceedings of the National Conference on Artificial
		  Intelligence (AAAI)} }
@STRING{accv	= {Proceedings of the Asian Conference on Computer Vision
		  (ACCV)} }
@STRING{acl	= {Proc. of the Annual Meeting of the Association of
		  Computational Linguistics (ACL)} }
@STRING{ai	= {Artificial Intelligence} }
@STRING{aistat	= {Proceedings of the International Workshop on Artificial
		  Intelligence and Statistics (AISTAT)} }
@STRING{anlp	= {Proceedings of the ACL Conference on Applied Natural
		  Language Processing} }
@STRING{arpa	= {Proceedings of the ARPA Workshop on Human Language
		  Technology} }
@STRING{benjamin= {Benjamin/Cummings Publishing Company, Inc.} }
@STRING{cacm	= {Communications of the ACM} }
@STRING{cambridge={Cambridge University Press} }
@STRING{cl	= {Computational Linguistics} }
@STRING{coling	= {Proc. the International Conference on Computational
		  Linguistics (COLING)} }
@STRING{colt	= {Proceedings of the Annual ACM Workshop on Computational
		  Learning Theory (COLT)} }
@STRING{conll	= {Proceedings of the Annual Conference on Computational
		  Natural Language Learning (CoNLL)} }
@STRING{csl	= {Computer Speech and Language} }
@STRING{cvpr	= {Proceedings of the IEEE Conference on Computer Vision and
		  Pattern Recognition (CVPR)} }
@STRING{eccv	= {Proceedings of the European Conference on Computer Vision
		  (ECCV)} }
@STRING{ecml	= {Proceedings of the European Conference on Machine Learning
		  (ECML)} }
@STRING{emnlp	= {Proc. of the Conference on Empirical Methods for Natural
		  Language Processing (EMNLP)} }
@STRING{focs	= {Proceedings of the IEEE Symposium of Foundation of
		  Computer Science (FOCS)} }
@STRING{iaai	= {Proceedings of the National Conference on Innovative
		  Applications of Artificial Intelligence (IAAI)} }
@STRING{icassp	= {Proceedings of the ICASSP} }
@STRING{icml	= {Proceedings of the International Conference on Machine
		  Learning (ICML)} }
@STRING{ijcai	= {Proceedings of the International Joint Conference on
		  Artificial Intelligence (IJCAI)} }
@STRING{ijcnlp	= {Proc. of the International Joint Conference on Natural
		  Language Processing (IJCNLP)} }
@STRING{infctrl	= {Information and Control} }
@STRING{ismb	= {Proceedings of the International Conference on Intelligent
		  Systems for Molecular Biology (ISMB)} }
@STRING{it	= {IEEE Transactions on information theory} }
@STRING{jacm	= {Journal of the ACM} }
@STRING{jair	= {Journal of AI Research} }
@STRING{jmlr	= {Journal of Machine Learning Research} }
@STRING{mit	= {MIT Press} }
@STRING{ml	= {Machine Learning} }
@STRING{mm	= {IEEE Transactions on Multimedia} }
@STRING{naacl	= {Proc. of the Annual Meeting of the North American
		  Association of Computational Linguistics (NAACL)} }
@STRING{neurips	= {Proceedings of the Conference on Advances in Neural
		  Information Processing Systems (NeurIPS)} }
@STRING{nips	= {Proceedings of the Conference on Advances in Neural
		  Information Processing Systems (NeurIPS)} }
@STRING{nle	= {Journal of Natural Language Engineering} }
@STRING{pami	= {IEEE Transactions on Pattern Analysis and Machine
		  Intelligence} }
@STRING{sigdat	= {Proceedings of the Conference on Empirical Methods for
		  Natural Language Processing (EMNLP)} }
@STRING{sigir	= {Proceedings of the International Conference on Research
		  and Development in Information Retrieval (SIGIR)} }
@STRING{sijad	= {SIAM Journal of Algebraic and Discrete Methods} }
@STRING{sijc	= {SIAM Journal of Computing} }
@STRING{stoc	= {Proceedings of the ACM Symposium of the Theory of
		  Computing (STOC)} }
@STRING{tassp	= {IEEE Transactions on Acoustics, speech, and Signal
		  Processing} }
@STRING{tassp	= {IEEE Transactions on Acoustics, speech, and Signal
		  Processing} }
@STRING{tcs	= {Theoretical Computer Science} }
@STRING{uai	= {Proceedings of the Conference on Uncertainty in Artificial
		  Intelligence (UAI)} }
@STRING{www	= {Proceedings of the International World Wide Web Conference
		  (WWW)} }
		  
@inproceedings{bolukbasi2016man,
  title={Man is to computer programmer as woman is to homemaker? debiasing word embeddings},
  author={Bolukbasi, Tolga and Chang, Kai-Wei and Zou, James Y and Saligrama, Venkatesh and Kalai, Adam T},
  booktitle= neurips,
  year={2016}
}
